Video Compression Beyond VVC: Quantitative Analysis of Intra Coding Tools in Enhanced Compression Model (ECM)

A quantitative analysis of post-VVC luma and chroma intra tools is presented, focusing on their statistical behaviors, in terms of block selection rate under different conditions. The aim is to provide insights to the standardization community, offering a clearer understanding of interactions between tools and assisting in the design of an optimal combination of these novel tools when the JVET enters the standardization phase. Specifically, this paper examines the selection rate of intra tools as function of 1) the version of the ECM, 2) video resolution, and 3) video bitrate. Additionally, tests have been conducted on sequences beyond the JVET CTC database. The statistics show several trends and interactions, with various strength, between coding tools of both luma and chroma.

==> figs/perf_class.tex <==
  \begin{tabular}{|c|c|c|c|}
    \hline
    Class & Y & Cb & Cr  \\
    \hline
    Class A1 &-10.8 \%&	-21.8 \%&	-29.3 \% \\
    \hline
    Class A2 & -17.0 \%&	-28.8 \%&	-31.8 \% \\
    \hline
    Class B & -11.3 \%&	-26.9 \%&	-25.0 \% \\
    \hline
    Class C & -11.4 \%&	-16.7 \%&	-17.2 \% \\
    \hline
    Class E & -15.0 \%&	-24.8 \%&	-23.1 \% \\
    \hline
    \textbf{Overall} & \textbf{-12.81 \%}&	\textbf{-23.73 \%}&	\textbf{-24.81 \%} \\
    \hline
    Class D & -9.5 \%&	-14.6 \%&	-14.7 \% \\
    \hline
  \end{tabular}
